Exploiting the Uncertainty of the Longest Paths: Response Time Analysis for Probabilistic DAG Tasks

Parallel real-time systems (e.g., autonomous driving systems) often contain functionalities with complex dependencies and execution uncertainties, leading to significant timing variability which can be represented as a probabilistic distribution. However, existing timing analysis either produces a single conservative bound or suffers from severe scalability issues due to the exhaustive enumeration of every execution scenario. This causes significant difficulties in leveraging the probabilistic timing behaviours, resulting in sub-optimal design solutions. Modelling the system as a probabilistic directed acyclic graph (p-DAG), this paper presents a probabilistic response time analysis based on the longest paths of the p-DAG across all execution scenarios, enhancing the capability of the analysis by eliminating the need for enumeration. We first identify every longest path based on the structure of p-DAG and compute the probability of its occurrence. Then, the worst-case interfering workload is computed for each longest path, forming a complete probabilistic response time distribution with correctness guarantees. Experiments show that compared to the enumeration-based approach, the proposed analysis effectively scales to large p-DAGs with computation cost reduced by six orders of magnitude while maintaining a low deviation (1.04% on average and below 5% for most p-DAGs), empowering system design solutions with improved resource efficiency.

==> old_files/intro_old.tex <==
% \vspace{-.4em}



% The cp-task releases an infinite sequence of instances noted as \textit{jobs}. The i-th job of the task is denoted as $G_i$. The response time of $G_i$ is:
% \begin{equation}
%     R(G_i) \leq len(G) + \frac{1}{m}(vol(G) - len(G)) + \max\{0, R(G_{i - 1}) - D(G_{i - 1})\}
% \end{equation}

% assume $\Gamma_i$ denotes the distribution of the path length from $v_{src}$ to $v_i$, each \textit{element} $e_i$ in the distribution is represented by a \textit{length} $l_i$ and $prob_i$, while the sum of $prob_i$ is equal to 1.

% \parlabel{Probability in parameters.}
% The presence of conditional branches changes some of the parameters of the system from a single value to a probability distribution. Take $len(\lambda)$ for example, three main cases can be summarized:
% \begin{itemize}
%     \item [1)] In the case of two regular nodes with a dependency, the WCET of the node can be added directly, as illustrated in Fig.\ref{seq}.
%     \item [2)] The case of two regular nodes with a shared successor, as illustrated in Fig.\ref{reg}.
%     \item [3)] The case of two conditional nodes with a shared $v_{ext}$, as illustrated in Fig.\ref{cond}.
% \end{itemize}

% \begin{figure}[htbp!]
% \centering
% \includegraphics[width=\linewidth]{figs/1.pdf}
% \caption{The sequential structure} \label{seq}
% \end{figure}

% \begin{figure}[htbp!]
% \centering
% \includegraphics[width=\linewidth]{figs/2.pdf}
% \caption{The regular fork structure} \label{reg}
% \end{figure}

% \begin{figure}[htbp!]
% \centering
% \includegraphics[width=\linewidth]{figs/3.pdf}
% \caption{The conditional fork structure} \label{cond}
% \end{figure}













\section{Introduction}
\label{sec:intro}

\gyynote{refine this section}

Our method aims to produce a distribution of response times for a heterogeneous soft real-time system, which reveals complete timing profiles in contrast to a single value (i.e., the worst case). To generate this distribution, we assume: ...

\parlabel{Background \& Motivation.}

With the complex functionalities implemented in real-time applications, directed acyclic graphs (DAGs) are widely used to model tasks with dependencies.
However, with the increasing complexity of real-world application scenarios (\eg, image processing and autonomous driving), the existence of conditional branches (such as if-then-else statements) and control flow introduces uncertainty in the execution of the DAG task. The characteristics (\eg the length of critical path and interference among paths) of a task may significantly vary depending on the particular instance, which amplifies the complexity of response time analysis. 

The application in image processing is as follows \cite{melani2015response}.
\begin{itemize}
    \item Fork a large number of sub-tasks to process small clusters of pixels in a parallel way.
    \item Run a single sub-task to process a larger sampled set of pixels sequentially.
\end{itemize}
Moreover, the level of detail at which each image region is processed may dynamically vary depending on runtime information. For example, when an object is detected in a particular region, the processing detail for the associated region may be progressively intensified, thus reducing the number of pixels to process.

Another example \cite{ueter2021response} is the size of images/videos in autonomous driving depends on varying sensor inputs, which is relevant to conditions such as weather or real-time road information.



\parlabel{Problem and Target.}

The existing analysis methods for the standard model cannot be applied to conditional branches directly because of the probabilistic execution behavior. Thus, the researchers have proposed the conditional DAG (C-DAG) task model and constructed the relevant analysis method.

The existing works \cite{melani2015response}, \cite{ueter2021response}, \cite{he2021response} focus on the worst-case of the response time and give the upper bound of the response time. However, these methods tend to pick the sub-branch with the most pessimistic execution expectation as the worst-case when calculating the response time. In fact, the conditional branch with the most pessimistic execution expectation may not be chosen frequently. For example in Fig.\ref{cdag}, as for the conditional node $v_2$, the upper branch with node $v_4$ in the path is the worst-case scenario with the maximum workload. However, the probability of the worst-case branch occurring is extremely low (0.1 in this example). For soft real-time applications, where occasional deadline misses are permissible, focusing solely on worst-case response times may amplify the pessimism in the schedulability analysis. Thus, \textbf{our target} is to propose a novel probabilistic response time analysis that accepts the uncertain execution behavior of the conditional DAGs.

\begin{figure}[htbp!]
\centering
\includegraphics[width=0.9\linewidth]{figs/cdag.png}
\caption{An example of CDAG} \label{cdag}
\end{figure}

\parlabel{Start points.}

As the starting points for research, the following criteria may be focused:
\begin{itemize}
    \item \textbf{The worst-case response time per job.} Take this as the upper bound. For each conditional node, the branch with the worst-case is chosen.
    \item \textbf{The probability distribution of response time.} It is also equal to the probability of a deadline miss. The state space of probabilistic response time is exponential level. How to reduce the complexity remains a problem.
    \item \textbf{The probability for k consecutive deadline misses.} The existing work \cite{ueter2021response} assumes the probabilities of DAG instances are independent. Therefore, the probabilities of k consecutive deadline misses can be standardized as the product of k independent probabilities of deadline misses, considering the maximum amount of unfinished work. Further, a corollary issue is that, assuming the previous $n$ ($0 < n < k$) deadline misses have been observed, how to prevent the occurrence of k deadline misses by adjusting service degradation (opting for the branch with lower workload and interference)?
\end{itemize}


\parlabel{Novelty.}

\begin{itemize}
    \item Propose a probability distribution model of response time for conditional DAGs, aimed at mitigating the pessimistic estimate for soft real-time applications.
    \item Provide the response analysis support for soft real-time applications.
    \item The guarantee for k-consecutive deadline misses.
\end{itemize}

\parlabel{Some simple ideas and problems to discuss.}

\begin{itemize}
    \item For each DAG task, calculate the worst-case response time first. If the worst-case response time can meet the deadline, then no further probabilistic analysis is needed. Otherwise, we process the probabilistic response time analysis.
    % \item The analysis on k-consecutive deadline misses is node level or job level?
    \item As the probabilities for each branch change gradually, what is the influence of this on our analysis?
    \item How does the deadline miss guide the following jobs? Artificially adjusted to lower-loaded branches to guarantee the completion of the task? A simple idea is to select the branch with the lowest workload and interference to guarantee that $R \leq D$. Currently, two potential strategies are under consideration for handling service degradation: 1) Priority-based branch switching: This strategy involves sorting the conditional nodes in ascending order of priority and sequentially switching branches in that order. The primary advantage of this approach is that it ensures the execution of high-priority nodes, prioritizing their completion properly. 2) Response time reduction-based intervention: This strategy calculates the potential reduction in response time that would result from switching to lower branches for each conditional node. It then prioritizes interventions on the nodes with the most significant reductions. The advantage of this method is that it aims to maximize the number of nodes that can be executed successfully without artificial switching, ensuring broader system performance.
    % Currently, two possible strategies are considered: 1) sort the set of conditional nodes in ascending priority order, and artificially switch the branch in order. The advantage of doing this is to guarantee the nodes with higher priorities can be executed normally. 2) The other idea is to calculate the reduction in response time of switching lower branches for each conditional node and prioritize interventions on nodes with large reductions. The advantage of doing this is to guarantee that as many nodes as possible can execute properly.
    \item How to reduce the exponential level state space caused by the multiple branches? Can we use statistical characteristics to abstract the Volume and Length? A naive idea is that for each node with more than k probabilistic values, only the values corresponding to the largest k probabilities and the maximum values are retained. k can be set to a parameter that is positively correlated with the number of c-nodes and the number of branches (to be discussed further).
    As the example in Fig.\ref{conv}, after the convolution of two sets of probability values, there are five distinct probabilities. If we set $k=2$, then the first 2 probabilities and the maximum value will be retained, \ie, $25$, $35$, and $40$ in the figure. However, this doesn't mean the left values will be discarded. Instead, the probability of each value will be added to the probability corresponding to the first value larger than it. For example, the probability $0.06$ of value $30$ will be added to the probability of value $35$. The advantage of doing this is to reduce the complexity of the task without unduly amplifying the level of pessimism.
    \item How to deal with the uncertain interference from the conditional branches? If we apply the strategy above, then the size of uncertainty is no more than $k$.
    \item How to associate k-consecutive deadline misses with probabilistic response time?
\end{itemize}

\begin{figure}[htbp!]
  \centering
  \includegraphics[width=0.8\linewidth]{figs/convolution.drawio.pdf}
  \caption{Illustration}
  \label{conv}
\end{figure}

==> old_files/old.tex <==
\section{Identify the critical path}

The existence of conditional nodes exhibiting probabilistic execution, \ie, chose one branch to execute based on the current condition status. The uncertainty of the conditions introduces variability to the critical path.
In this section, we define the distribution of the critical paths within condition DAG to capture the probabilistic behavior of the conditional nodes.

To facilitate analysis, we categorize the paths based on the types of nodes they contain.
For clarity, we segregate the nodes into two mutually exclusive sets: the sets of regular and conditional nodes as $V_r$ and $V_c$, respectively.

\textit{Definition 1 (Regular Path).}
A regular path $\lambda_r = \{ v_0, \cdots, v_k \}$ is a set of nodes, where $\forall i \in \left[ 0, k - 1 \right]$, $v_i$ is the predecessor of $v_{i + 1}$; and $\forall j \in \left[ 0, k \right]$, $ v_j \in V_j$.

Regular paths consist exclusively of regular nodes and possess a unique length, as the execution of all nodes within the path is guaranteed.

\textit{Definition 2 (Conditional Path).}
A conditional path $\lambda_c = \{ v_0, \cdots, v_k \}$ is a set of nodes, where $\forall i \in \left[ 0, k - 1 \right]$, $v_i$ is the predecessor of $v_{i + 1}$; and $\exists j \in \left[ 0, k \right]$, $ v_j \in V_c$.

The conditional path contains at least one conditional node, which introduces probabilistic uncertainty to the path. Since the execution of the conditional nodes depends on the actual conditions, the conditional path is not guaranteed to be executed in each job.
% (may be used later) Consequently, we assign a probability to each conditional path, representing the likelihood of its execution in any given job. This probability is associated with the conditional nodes involved, and further details will be provided in the following sections.

Fig.\ref{figs:example} gives an example of conditional DAG, where the rectangle denotes the regular nodes, and the diamond (resp. circle) denotes the entry (resp. exit) of the conditional structure.
Each node is assigned a WCET (worst-case execution time) indicated by a red number, and the blue number denotes the probability of each branch being chosen.
There are two critical paths in the DAG, where the regular path $\lambda_r = \{ v_{src}, v_1, v_2, v_3, v_{snk} \}$ is with the length of 75, and the conditional path $\lambda_c = \{ v_{src}, v_4, v_5, v_7, v_8, v_9, v_{11} v_{snk} \}$ is with the length of 80.

\begin{figure}[http!]
\centering
\includegraphics[width=\linewidth]{figs/subfig.drawio.pdf}
\caption{An example of critical paths} \label{figs:example}
\end{figure}

% motivation
% \gyynote{motivation of our method}
% The motivation is ...


 
% 不同情况组合的复杂性/不同情况具体如何处理
% Overall, the longest length of the path between two nodes
% The distribution of critical paths can be described as finding the distribution of the longest paths between $v_{snk}$ and $v_{src}$. Thus, we can start by finding the distance distribution between two nodes, and 
% Finding the distribution of the critical path can be described as finding the longest path distribution between two nodes, while the target is to find the longest path distribution from $v_{snk}$ to $v_{src}$.

Essentially, determining the distribution of the critical path is equivalent to finding the distribution of the longest path from $v_{snk}$ to $v_{src}$.
Thus the problem can be reformulated as finding the distribution of the longest path between two given nodes.
The distribution of critical paths is then obtained through iteratively merging the distributions of neighboring paths.

% \textit{Definition 3 (Node Pair).}
% For two given nodes $v_i$ and $v_j$, the node pair is defined as $(v_i,v_j)$ if there exists a path from $v_i$ to $v_j$. $v_i$ and $v_j$ serve as the start node and end node, respectively.

%  = <v_i, v_j, \lambda_k>
\textit{Definition 3 (Path Distribution).}
The \textit{Path Distribution} is defined as $\pi_{i,j,k} = \{ l_k, prob_k \}$, capturing the probabilistic characteristics along the path $\lambda_k$ from $v_i$ to $v_j$, characterized by its length $l_{k}$ and a probability $prob_k$, which is determined by the conditional branches it incorporates.

\textit{Definition 4 (Blocks).}
The \textit{Blocks} is defined as $Block(i,j) = \{ v_k | v_k \in anc(v_j) \wedge v_k \in des(v_i) \}$, which denotes all the nodes between $v_i$ and $v_j$.

\textit{Definition 5 (Maximum Distance Distribution).}
The \textit{Maximum Distance Distribution (MDD)} is defined as $\Pi_{i,j}$, capturing the probabilistic characteristics of $Block(i,j)$. Each element $\pi_{i,j,k}$ in $\Pi_{i,j}$ represents the path $\lambda_k$ between the nodes. Especially, if all the paths from $v_i$ to $v_j$ are regular nodes, the MDD will only contain one element, while the corresponding probability is equal to 1.

\parlabel{Rules for distributions of critical paths.}

\textit{Scenario 1 (Path Concatenation).}
For the two MDD $\Pi_{i,j}$ and $\Pi_{j,k}$, where $v_j$ serves as the end node of the first MDD and the start node of the second one. The two MDDs can be concatenated into a longer one $\Pi_{i,k}$. The rules of three possible conditions are given as follows.

\textit{Rule 1 (Concatenation of regular blocks).}
For the blocks with regular nodes only, \ie, $\Pi_{i,j} = \{ \pi_{i,j,m} \}$ and $\Pi_{j,k} = \{ \pi_{j,k,n} \}$. The new MDD can be formulated by: $\Pi_{i,k} = \{ \pi_{i,k,t} \}$, where $\lambda_t = \lambda_m \cup \lambda_n$, $l_t = l_m + l_n$ and $prob_t = 1$.


\textit{Rule 2 (Concatenation of conditional blocks).}
For the two conditional blocks share a connected vertex, \ie, $\Pi_{i,j}$ and $\Pi_{j,k}$ with $v_j$ connected. Thus the new MDD $\Pi_{i,k}$ can be formulated as follows.
\begin{equation}
\begin{split}
    \Pi_{i,k} &= \{ \{ l_{k_1} + l_{k_2}, prob_{k_1} \cdot prob_{k_2} \} \\
    &| \{ l_{k_1}, prob_{k_1} \} \in \Pi_{i,j} \wedge \{ l_{k_2}, prob_{k_2} \} \in \Pi_{j,k} \}
\end{split}
\end{equation}
Here, each element in $\Pi_{i,k}$ represents a concatenated path. Its length consists of the combined lengths from $\Pi_{i,j}$ and $\Pi_{j,k}$. The associated probability is obtained by multiplying the probabilities of the contributing paths ($prob_{k_1} \cdot prob_{k_2}$).
% For the two conditional blocks with a connected vertex, \ie, $\Pi_{i,j}$ and $\Pi_{j,k}$ with $v_j$ connected. Thus the new MDD can be formulated by: $\Pi_{s,e}$, while for each $\pi_{a,b,k_1} \in \Pi_{a,b}$ and $\pi_{m,n,k_2} \in \Pi_{m,n}$, a new element $\pi_{s,e,k}$ is combined, where $\lambda_k = \lambda_{k_1} \cup \lambda_{k_2} \cup v_s \cup v_e$, $l_k = l_{k_1} + l_{k_2} + C_s + C_e$ and $prob_k = prob_{k_1} \cdot prob_{k_2}$.

\textit{Rule 3 (Concatenation of conditional block and regular block).}
Assuming the combination of a regular MDD $\Pi_{i,j} = \{ \pi_{i,j,m} \}$ and a conditional MDD $\Pi_{j,k}$, where $v_j$ is the connection of the two blocks. The $l_m$ from $\pi_{i,j,m}$ is the length of the path that the task will definitely execute.
Leveraging the sequential execution of these blocks and the fixed characteristics of the regular block, the longer MDD $\Pi_{i,k}$ can be calculated by:
\begin{equation}\label{conbine of cond and regular}
    \Pi_{i,k} = \{ \{ l_t + l_m, prob_t \} | \{ l_t, prob_t \} \in \Pi_{j,k} \}
\end{equation}
In Eq.\ref{conbine of cond and regular}, each element in $\Pi_{i,k}$ represents a combined path. Its length is computed by adding the length of the path from $\Pi_{j,k}$ (conditional blocks) to $l_m$ (regular blocks). The associated probability ($prob_t$) is directly taken from the corresponding element in $\Pi_{j,k}$. This equation efficiently calculates the combined distribution based on the properties of the individual blocks.
% Due to the two blocks being executed in sequence while the properties of the regular blocks are fixed, the new MDD, $\Pi_{i,k}$ can be derived from:
% The $l_m$ from $\pi_{i,j,m}$ is the length of the path that the task will definitely execute. Thus, the $l_m$ can be considered as a threshold to 

\gyynote{Give an example here}
\textit{Example 1:}

% For the two conditional paths, both the path distributions $\pi_{i,j,m}$ and $\pi_{j,k,n}$ are with $prob_m = 1 \wedge prob_n = 1$. Thus the new path distribution can be formulated by: $\pi_{i,j,k}$, where $\lambda_k = \lambda_m \cup \lambda_n$, $l_k = l_m + l_n$ and $prob_k = 1$.


\textit{Scenario 2 (Multiple Paths Integration).}
For the node pair with two or more blocks connected, \ie, $\Pi_{a,b}$ and $\Pi_{m,n}$ which represent two different blocks, where $v_a \in suc(v_i) \wedge v_m \in suc(v_i) \wedge v_b \in pre(v_j) \wedge v_n \in pre(v_j)$. Based on the two blocks, a new MDD of $Block(i,j)$ from $v_i$ to $v_j$ can be updated which incorporates the information from the two different sub-Blocks. The principles can be summarized as follows.

% For the node pair with two or more paths connected, \ie, $\lambda_1 = \{ v_i, \cdots, v_m, \cdots, v_j \}$ and $\lambda_2 = \{ v_i, \cdots, v_n, \cdots, v_j \}$ represent two different paths from $v_i$ to $v_j$, with $\Gamma_{}$.

\textit{Rule 4 (Parallelism of regular blocks).}
For the blocks with regular nodes only in pararell, \ie, $\Pi_{a,b} = \{ \pi_{a,b,x} \}$ and $\Pi_{m,n} = \{ \pi_{m,n,y} \}$. The new MDD can be formulated by: $\Pi_{i,j} = \{ \pi_{i,j,t} \}$, where $l_t = \max \{ l_x, l_y \} + C_i + C_j$ and $prob_t = 1$.

\textit{Rule 5 (Parallelism of conditional blocks).}
For the two block with conditions in parallel, \ie, $\Pi_{a,b}$ and $\Pi_{m,n}$, the new MDD $\Pi_{i,j}$ can be calculated as follows:
\begin{equation}
\begin{split}
    \Pi_{i,k} &= \{ \{ \max (l_x + l_y), prob_x \cdot prob_y \} \\
    & | \{ l_x, prob_x \} \in \Pi_{a,b} \wedge \{ l_y, prob_y \} \in \Pi_{m,n} \}
\end{split}
\end{equation}
Here, each element in $\Pi_{i,j}$ represents a combined path constructed by taking the maximum length ($l_x$ or $l_y$) and the product of probabilities ($prob_x$ and $prob_y$) from corresponding elements in $\Pi_{a,b}$ and $\Pi_{m,n}$. Intuitively, the maximum length reflects the dominance of the longer path, while the product of probabilities represents the joint occurrence of both elements.

% Intuitively, that each block indicates a distribution from $v_i$ to $v_j$, where the distributions of different blocks are mutually independent. Thus, we can iterate each element from the blocks, take the maximum length of the two blocks as the length that dominance, and take the product of probabilities as the probability that both elements happen.

% The calculation iterates through each element in both blocks, combining them into new elements with the maximum length and the product of probabilities. Intuitively, the maximum length reflects the dominance of the longer path, while the product of probabilities represents the joint occurrence of both elements.

% Taking the maximum length captures the worst-case scenario where the longer path dominates while multiplying probabilities yields the overall likelihood of both conditions being met.
% Therefore, we iterate over each element pair from the blocks, selecting the maximum length for dominance and multiplying the probabilities to account for the combined event of both elements occurring.


\textit{Rule 6 (Parallelism of conditional blocks and regular blocks).}
Consider the scenario where a regular MDD $\Pi_{a,b} = \{ \pi_{a,b,t} \}$ and a conditional MDD $\Pi_{m,n}$ are combined to represent the distribution between $v_i$ and $v_j$. The $l_t$ from $\pi_{a,b,t}$ represents the deterministic length of a path guaranteed to be executed by the task. Leveraging this information, we can utilize $l_t$ as a threshold to selectively prune elements from $\Pi{m,n}$ and obtain a more accurate distribution.
% Thus, the $l_m$ can be considered as a threshold to prune $\Pi_{m,n}$ and form a more accurate distribution.
\begin{equation}\label{mix parallel}
\begin{split}
    \Pi_{i,j} = \bigcup_{\pi_{x,y,k} \in \Gamma} \{ &\pi_{x,y,k} \} \cup \{ l_t, prob_{const} \} \\
    \Gamma = \{ \{ l_k + C_i + C_j, prob_k  \} &| \{ l_k, prob_k \} \in \Pi_{m,n} \wedge l_k > l_t \} \\
    prob_{const} = &\sum\limits_{\substack{ \{ l_r, prob_r \} \in \Pi_{m,n}, \\ l_r \leq l_t}} prob_r
\end{split}
\end{equation}
Where, $\Gamma$ represents the subset of elements from $\Pi_{m,n}$ where the path length exceeds the lower bound $l_t$.
These elements are combined with the threshold length $l_t$ and a constant probability $prob_{const}$, which aggregates the probabilities of all paths in $\Pi_{m,n}$ shorter than $l_t$, demonstrating the dominance over these paths.

% In Eq.\ref{mix parallel}, the length of regular block $l_t$ serves as a lower bound to prune the elements in $\Pi_{m,n}$ with shorter path length, while the sum of these elements is considered as the probability of $l_t$.

\parlabel{Algorithm.}

% \begin{algorithm}[htbp!]
% \caption{Distributions of Critical Paths}\label{critical paths}
% \KwIn{$C_{t}$, $\mathcal{P}$, $Exe$}

% $COG = \{\}$\;

% \For{$p \in \mathcal{P}$}{
%     \If{$p$ is busy}{
%         $COG = COG \cup Exe(p)$\;
%     }
% }

% $F_t = \{\}$\;
% \For{$v_i \in COG$}{
%     \For{$v_j \in suc(v_i)$}{
%         \If{$v_j \notin F_t$}{
%             Flag\ =\ true\;
%             \For{$v_k \in pre(v_j)$}{
%                 \If{$v_k \notin COG$ and $v_k$ haven't been finished}{
%                     Flag\ =\ false\;
%                     break\;
%                 }
%             }
%             \If{Flag}{
%                 $F_t = F_t \cup v_j$\;
%             }
%         }
%     }
% }
% \end{algorithm}
